A Distributed and Deterministic TDMA Algorithm for Write-All-With-Collision Model

Several self-stabilizing time division multiple access (TDMA) algorithms are proposed for sensor networks. In addition to providing a collision-free communication service, such algorithms enable the transformation of programs written in abstract models considered in distributed computing literature into a model consistent with sensor networks, i.e., write all with collision (WAC) model. Existing TDMA slot assignment algorithms have one or more of the following properties: (i) compute slots using a randomized algorithm, (ii) assume that the topology is known upfront, and/or (iii) assign slots sequentially. If these algorithms are used to transform abstract programs into programs in WAC model then the transformed programs are probabilistically correct, do not allow the addition of new nodes, and/or converge in a sequential fashion. In this paper, we propose a self-stabilizing deterministic TDMA algorithm where a sensor is aware of only its neighbors. We show that the slots are assigned to the sensors in a concurrent fashion and starting from arbitrary initial states, the algorithm converges to states where collision-free communication among the sensors is restored. Moreover, this algorithm facilitates the transformation of abstract programs into programs in WAC model that are deterministically correct.

==> concl.tex <==
\section{Conclusion}
\label{sec:concl}

In this paper, we presented a self-stabilizing deterministic TDMA slot assignment algorithm for write all with collision (WAC) model. We showed that the algorithm allows sensors to concurrently recover and self-stabilize starting from arbitrary states. Towards this end, we used distributed reset to restore the state of the network quickly. More specifically, whenever a sensor observes a collision for a threshold number of consecutive TDMA frames, it schedules a reset computation to recover its distance 2 neighborhood. We showed that at most one reset operation executes in a distance 3 neighborhood at any instant. And, we showed how the sensors recover in response to resets and reach legitimate states that satisfy the problem statement of TDMA.  

Additionally, as discussed in \cite{ka06a}, our algorithm is applicable in transforming existing programs in shared memory model into programs in WAC model. This allows one to reuse existing solutions in distributed computing for problems such as routing, data dissemination, synchronization, and leader election in the context of sensor networks. Thus, the algorithm proposed in this paper allows one to transform such solutions and evaluate them in sensor networks. As a result, we can rapidly prototype sensor network applications. (We refer the reader to \cite{arumugam-dissertation06} for examples of such transformations.) Moreover, this algorithm demonstrates the feasibility of a deterministic transformation of a program in shared memory model into a program in WAC model while preserving the self-stabilization property of the original program. 

There are several possible future directions. While this algorithm demonstrates concurrent recovery of TDMA slots and the recovery time is expected to be reasonable for typical deployments, one future direction is to extend this algorithm to provide faster convergence. Additionally, while our experience in transformation of abstract programs to WAC model (cf. \cite{arumugam-dissertation06}) suggests that the efficiency of the program obtained by transformation is close to that of manually designed programs, another future direction is to quantify the efficiency of the transformed programs.



==> intro.tex <==
\section{Introduction}
\label{sec:intro}

One of the important concerns in programming distributed computing platforms is the model of computation used to specify programs. Programs written for distributed computing platforms such as sensor networks and embedded systems often have to deal with several low level challenges of the platform. In sensor networks, especially, one has to write programs that deal with issues such as communication, message collision and race conditions among different processes. Therefore, to simplify the programming, it is important to abstract such low level issues. In other words, the ability to specify programs in an abstract model and later transform them into a concrete model that is appropriate to the platform is crucial. 

The problem of transformation of programs in an abstract model to programs in other models of computation has been studied extensively (e.g., \cite{as99, gh97, gh99, kio+02, ky02, na02}). These transformations cannot be applied to obtain concrete programs for sensor networks as the model of computation in sensor networks is {\em write all with collision} (WAC) model. In WAC model, communication is {\em local broadcast} in nature. As a result, whenever a sensor executes an {\em action}, it writes the state of all its neighbors in one atomic step. However, if two neighbors $j$ and $k$ of a sensor (say $i$) try to execute their write actions at the same time then, due to collision, state of $i$ will remain unchanged. The actions of $j$ and $k$ may update the state of their other neighbors successfully. 

\noindent{\bf Existing transformations for WAC model. } \
Recently, several approaches have been proposed to transform programs written in abstract models considered in distributed computing literature into programs in WAC model \cite{herman03, ht04, ka06a, ak06jacic}. Such transformation algorithms can be classified into two categories: (a) randomized \cite{herman03, ht04} and (b) deterministic \cite{ka06a, ak06jacic}.

In \cite{herman03}, the authors propose a {\em cached sensornet transform} (CST) that allows one to correctly simulate an abstract program in sensor networks. This transformation uses carrier sensor multiple access (CSMA) based MAC protocol to broadcast the state of a sensor and, hence, the transformed program is randomized. And, the algorithm in \cite{ka06a} uses time division multiple access (TDMA) to ensure that collisions do not occur during write actions. Specifically, in WAC model, each sensor executes the {\em enabled} actions in the TDMA slots assigned to that sensor. And, the sensor writes the state of all its neighbors in its TDMA slots. If the TDMA algorithm in \cite{ka06c}, a self-stabilizing and deterministic algorithm designed for grid-based topologies, is used with \cite{ka06a} then the transformed program in WAC model is self-stabilizing and deterministically correct for grid-based topologies. And, if randomized TDMA algorithms proposed in \cite{ht04,bms+04} are used with \cite{ka06a} then the transformed program is probabilistically correct. Finally, the algorithm in \cite{ak06jacic}, a self-stabilizing and deterministic TDMA algorithm for arbitrary topologies, allows one to transform abstract programs into programs in WAC model that are deterministically correct for arbitrary topologies.

In this paper, we are interested in stabilization preserving deterministic transformation for WAC model. As mentioned above, a self-stabilizing deterministic TDMA algorithm enables such a transformation. One of the drawbacks of existing self-stabilizing deterministic TDMA algorithms (e.g., \cite{ak06jacic}) is that the recovery is sequential. Specifically, in \cite{ak06jacic}, whenever the network is perturbed to states where the TDMA slots are not collision-free, a distinguished sensor (e.g., base station) initiates a recovery process and each sensor recomputes its slots one by one. However, it is desirable that the network self-stabilizes from such arbitrary states in a distributed and concurrent manner (without the assistance of distinguished sensors). 

\noindent{\bf Contributions of the paper. } \
To redress this deficiency, in this paper, we propose a self-stabilizing deterministic TDMA algorithm that provides concurrent recovery. In this algorithm, whenever a sensor observes that the slots assigned to its neighbors are not collision-free, it initiates a recovery. As a result, its neighbors recover to legitimate states (i.e., the slots are collision-free) and the network as a whole self-stabilizes concurrently. We show that the algorithm supports addition or removal of sensors in the network. While a removal of a sensor does not affect the normal operation of the network, our algorithm ensures that the slots assigned to removed sensor are reused. And, our algorithm supports {\em controlled} addition of new sensors in the network. In addition, we propose an extension to our algorithm that improves the bandwidth allocation of the sensors. 

\noindent{\bf Organization of the paper. } \ 
The rest of the paper is organized as follows. In Section \ref{sec:prelims}, we introduce the models of computation considered in distributed computing platforms. We formally state the problem definition of TDMA and identify the assumptions made in this paper. In Section \ref{sec:algo_wac}, we present our distributed TDMA slot assignment algorithm for WAC model. We show that the algorithm is self-stabilizing. Also, we discuss extensions that allow dynamic addition/removal of sensors, improve bandwidth allocation, and synchronize time. Then, in Section \ref{sec:rel}, we compare our algorithm with related work. Finally, in Section \ref{sec:concl}, we summarize our work and identify future research directions.


==> related.tex <==
\section{Related Work}
\label{sec:rel}

Related work that deals with self-stabilizing deterministic slot assignment algorithms include \cite{ak06jacic,ka06c,dnt06,rr05}. In \cite{ka06c}, Kulkarni and Arumugam proposed self-stabilizing TDMA (SS-TDMA). In this algorithm, the topology of the network is known upfront and remains static. Also, a base station is responsible for periodic diffusing computations that assign/revalidate the slots of the sensors. Unlike \cite{ka06c}, in the proposed algorithm, the sensors are aware of only their neighbors and there is no designated sensor that is responsible for the slot assignment. 

In \cite{ak06jacic}, Arumugam and Kulkarni proposed self-stabilizing deterministic TDMA algorithm. Again, this algorithm assumes the presence of the base station that is responsible for token circulation. And, the slots are assigned in sequential fashion. By contrast, the algorithm proposed in this paper assigns slots in a concurrent fashion and no token circulation is required. 

In \cite{dnt06}, Danturi et al proposed a self-stabilizing solution to dining philosophers problem where a process cannot share the critical section (CS) with non-neighboring processes also. This problem has application in distance-k coloring, where $k$ is the distance up to which a process cannot share CS. This algorithm requires each process $p$ to maintain a tree rooted at itself that spans the processes with whom $p$ cannot share CS using algorithms in the literature. However, the algorithm is written in shared memory model. On the other hand, the proposed algorithm can be used in sensor networks directly and also allows one to transform abstract programs into programs in WAC model. 

In \cite{rr05}, BitMAC is proposed for collision-free communication in sensor networks. One of the important assumptions in this paper is that when two messages collide the result is an OR operation between them. This algorithm is not self-stabilizing. Unlike \cite{rr05}, our algorithm is written for WAC model and is self-stabilizing.

Related work that deals with randomized algorithms for TDMA slot assignment include \cite{ht04, bms+04}. In \cite{ht04}, Herman and Tixeuil proposed a probabilistic fast clustering technique for TDMA slot assignment. In this algorithm, first, a maximal independent set that identifies the leaders is computed. These leaders are then responsible for distance 2 coloring. In \cite{bms+04}, Busch et al proposed a randomized algorithm for slot assignment. The algorithm operates in two phases: (1) to compute the slots and (2) to determine the ideal TDMA period. Both these phases are self-stabilizing and can be interleaved. Unlike \cite{ht04,bms+04}, our algorithm is deterministic.

Several other TDMA algorithms are proposed in the literature (e.g., \cite{cls01,hcb02,sp99,ayy02}). However, most of these algorithms are not self-stabilizing and/or make assumptions that are not relevant to WAC model or sensor networks. 

